New methods for the computation of the linear response within the density functional theory in spin polarized system (Metodi innovativi per il calcolo della risposta lineare in density functional theory per sistemi spin polarizzati)

In the present thesis we study absorption spectra of spin polarized isolated systems. Thus we introduce the density functional theory (DFT) formalism and its time dependent extension (TDDFT) together with the approximation used. In particula the Casida formulation of TDDFT is described. The equations for the description of open shell systems have been implemented in the abinit code. Then we used the BeH molecule as a test case. Studying the results for this molecule we underline the limits of the commonly used approximations. In particular we discuss why the the spin symmetry of excited states is broken and we propose a rule to find which excitation energies are affected by this problem. Finally, in the last part, we discuss how a better approximation could be obtained starting from the many body perturbation theory. ----- Il lavoro della presente tesi \`e focalizzato sullo studio dello spettro di eccitazione di sistemi isolati spin polarizzati. Quindi vengono esposte la Density Functional Theory (DFT), la sua estensione al caso dipendente dal tempo (TDDFT) e le approssimazioni utilizzate. In particolare vien esposta la formulazione di Casida della TDDFT. Le equazioni per lo studio di sistemi spin-polarizzati sono state implementate all'interno del software ABINIT. \`E stata poi scelta la molecola di BeH per testare l'implementazione fatta. I calcoli eseguiti ci hanno permesso di mettere in luce i limiti delle approssimazioni comunemente utilizzate. In particolare abbiamo discusso l'impossibilit\`a di mantenere la corretta simmetria di spin in sistemi spin polarizzati. Viene quindi proposta una regola per individuare quali siano, negli spettri calcolati, le energie di eccitazione affette da questo problema. Nell'ultimo capitolo della tesi viene inoltre esposta una possibile soluzione per superare l'approssimazione adiabatica.

==> definizioni.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Parentesi per i le contrazioni
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\makeatletter
\def\overbracket{\@ifnextchar [ {\@overbracket} {\@overbracket
[\@bracketheight]}}
\def\@overbracket[#1]{\@ifnextchar [ {\@over@bracket[#1]}
{\@over@bracket[#1][0.3em]}}
\def\@over@bracket[#1][#2]#3{%\message {Overbracket: #1,#2,#3}
\mathop {\vbox {\m@th \ialign {##\crcr \noalign {\kern 3\p@
\nointerlineskip }\downbracketfill {#1}{#2}
                              \crcr \noalign {\kern 3\p@ }
                              \crcr  $\hfil \displaystyle {#3}\hfil $%
                              \crcr} }}\limits}
\def\downbracketfill#1#2{$\m@th \setbox \z@ \hbox {$\braceld$}
                  \edef\@bracketheight{\the\ht\z@}\downbracketend{#1}{#2}
                  \leaders \vrule \@height #1 \@depth \z@ \hfill
                  \leaders \vrule \@height #1 \@depth \z@ \hfill
\downbracketend{#1}{#2}$}
\def\downbracketend#1#2{\vrule depth #2 width #1\relax}
\makeatother
%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%Stile nell'impaginazione
%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\pagestyle{fancy}
\renewcommand{\chaptermark}[1]
             {\markboth{#1}{}}
\renewcommand{\sectionmark}[1]
             {\markright{\thesection\ #1}}
\fancyhf{}
\fancyhead[LE,RO]{\bfseries\thepage}
\fancyhead[LO]{\bfseries\rightmark}
\fancyhead[RE]{\bfseries\leftmark}
\renewcommand{\headrulewidth}{0.5pt}
\renewcommand{\footrulewidth}{0pt}
\addtolength{\headheight}{0.5pt}
\fancypagestyle{plain}{%
              \fancyhead{}
              \renewcommand{\headrulewidth}{0pt}}


==> intestazione.tex <==
\pagestyle{fancy}
\renewcommand{\chaptermark}[1]
             {\markboth{#1}{}}
\renewcommand{\sectionmark}[1]
             {\markright{\thesection\ #1}}
\fancyhf{}
\fancyhead[LE,RO]{\bfseries\thepage}
\fancyhead[LO]{\bfseries\rightmark}
\fancyhead[RE]{\bfseries\leftmark}
\renewcommand{\headrulewidth}{0.5pt}
\renewcommand{\footrulewidth}{0pt}
\addtolength{\headheight}{0.5pt}
\fancypagestyle{plain}{%
              \fancyhead{}
              \renewcommand{\headrulewidth}{0pt}}


==> kernel_fantom.tex <==
\section{L'equazione di S.S. per il kernel}

%************************************************************************************************

\subsection{Il "Nanoquanta Kernel"}

\begin{eqnarray}
\left[f_{xc}(\vec{r},t;\vec{r}',t') \right]_{\sigma,\tau} = 
\left[f_{xc}^{eff}(\vec{r},t;\vec{r}',t') \right]_{\sigma,\tau} + 
\left[f_{xc}^{(1)}(\vec{r},t;\vec{r}',t') \right]_{\sigma,\tau}      \\
\left[f_{xc}^{(1)}(\vec{r},t;\vec{r}',t') \right]_{\sigma,\tau} = 
\left[\chi_{0}^{-1}(\vec{r},t;\vec{r}',t') \right]_{\sigma,\tau}-
\left[\Pi_{0}^{-1}(\vec{r},t;\vec{r}',t') \right]_{\sigma,\tau}
\end{eqnarray}

If $\omega>0$ the retarded and the T-ordered functions are equal.
It would be interesting to understand what appens if we also consider
negative frequences and if it would be useful, within the approximations
done, try to solve the problem of the differences between this two
tipe of quantities.



Ref.[10]: "Many Body perturbation theory using density functional
concept: beyond GW approximation"



New set of Equations:

\begin{eqnarray} 
\label{eq:Hedin}
 &&G(1,2) = g(1,2) + g(1,3) \Sigma^{\star}(3,4) G(4,2)   \\
 &&W(1,2) = U_0(1,2) + U_0(1,3) \Pi^{\star}(3,4) W(4,2)   \\
 &&f_{xc}^{eff}(1,2) = -i \Pi_0^{-1}(1,5) G(5,4) G(3,5) 
                   \frac{\delta \Sigma^{\star}(4,3)}{\delta \rho(2)} \\
 &&\Gamma(1;2,3) = \delta(1,2)\delta(1,3)
               + \delta(2,3)f_{xc}^{eff}(2,4) \Pi(4,1) \nonumber \\
 &&            + \left( \frac{\delta \Sigma^{\star}(2,3)}{\delta \rho(4)}
               - \delta(2,3) f_{xc}^{eff}(2,4) \right) \Pi(4,1) \\ 
 &&\hbar \Pi^{\star}(1,2) = -2i \Gamma(1;3,4) G(2,3) G(4,2)     \\
 &&\hbar \Sigma^{\star}(1,2) = i \Gamma(4;1,3) G(3,2) W(4,2)
\end{eqnarray}
Possible scheme:

\begin{eqnarray}
 G(1,2)=g(1,2) ;\;\;\;
 \Gamma(1;2,3)=\delta(1,2) \delta(1,3)  ;\;\;\;
 W(1,2)=U_0 
\nonumber
\end{eqnarray}

\begin{eqnarray}
 &&\hbar \Pi^{\star}(1,2) = -2i \Gamma(1;3,4) G(2,3) G(4,2)    \\
 &&W(1,2) = U_0(1,2) + U_0(1,3) \Pi^{\star}(3,4) W(4,2)        \\
 &&\hbar \Sigma^{\star}(1,2) = i \Gamma(4;1,3) G(3,2) W(2,4)
\end{eqnarray}

\begin{eqnarray}
 f_{xc}^{eff}(1,2) &=& -i \Pi_0^{-1}(1,5) G(5,4) G(3,5) 
                   \frac{\delta \Sigma^{\star}(4,3)}
                        {\delta \rho(2)}                       \\
 \frac{\delta \Sigma^{\star}(4,3)}{\delta \rho(2)}
    &\approx& \frac{\delta \left[ G(4,3) W(4,3) \right]}
                   {\delta \rho(2)}                            \\ \nonumber
    &\approx& \frac{\delta G(4,3)}{\delta \rho(2)} W(4,3)      \\   \nonumber
    &=& G(4,6)\frac{G^{-1}(6,7)}{\delta \rho(2)} G(7,3) W(4,3) \\ \nonumber
    &\approx& G(4,6) \Pi_0^{-1}(6,2) G(6,3) W(4,3)             \\
 \Gamma(1;2,3) &\approx& \delta(1,2)\delta(1,3)
               + \delta(2,3)f_{xc}^{eff}(2,4) \Pi(4,1)
\end{eqnarray}
\begin{eqnarray}
 \Sigma^{\star}(1,2) &=& G(3,2) W(4,2) \Gamma(4;1,3)                   \\
 G(1,2) &=& g(1,2) + g(1,3) \Sigma^{\star}(3,4) G(4,2)
\end{eqnarray}


\begin{itemize}
\item The following approximation are involved in the functional derivative
of $\Sigma^{\star}$:
\begin{enumerate}
\item we use $\Sigma^{\star}=GW$ so that vertex corrections are
      neglected there
\item we neglect $\frac{\delta W}{\delta \rho}G$ there
\item the functional derivative of $G^{-1}$ respect to $\rho$ is
      approximated to $\Pi_0^{-1}$, so that we neglect there the functional
      derivative of $\Sigma^{\star}$. The right expression would be:
      $\frac{\delta G^{-1}}{\delta \rho}=\Pi_0^{-1}
      +\frac{\delta \Sigma^{\star}}{\delta \rho}$
\end{enumerate}
\item The following approximation is used for $\Gamma$:
\begin{enumerate}
\item We neglected the term 
      $\left(\frac{\delta \Sigma^{\star}}{\delta \rho}-\delta
       f_{xc} \right) \Pi_o^{-1}$
\end{enumerate}
\end{itemize}


Let's write the equations in a more explicit way,
that is: $1=(\vec{x}_1,t_1,\sigma_1)$

\begin{eqnarray}
&& \left[f_{xc}^{eff}(\vec{x},t_x;\vec{y},t_y) \right]_{\sigma,\tau}
   = -i \left[\Pi_0^{-1}(\vec{x},t_x;\vec{z}_1,t_1)
        \right]_{\sigma,\eta_1}*                              \\  \nonumber
&&    *G_{\eta_1,\eta_2}(\vec{z}_1,t_1;\vec{z}_2,t_2)       
       G_{\eta_3,\eta_1}(\vec{z}_3,t_3;\vec{z}_1,t_1)
     \frac{\delta \Sigma^{\star}_{\eta_2,\eta_3}
       (\vec{x}_2,t_2;\vec{z}_3,t_3)}
       {\delta \rho_{\tau}(\vec{y},t_y)}                      \\   
&& \frac{\delta \Sigma_{\sigma,\tau}^{\star}(\vec{x},t_x;\vec{y},t_y)}
        {\delta \rho_{\eta}(\vec{z},t_z)}
    \approx G_{\sigma,\mu_1}(\vec{x},t_x;\vec{u}_1,t_1)
    \left[\Pi_0^{-1}(\vec{u}_1,t_1;\vec{z},t_z) \right]_{\mu_1,\eta} \\ \nonumber
&&  G_{\mu_1,\tau}(\vec{u}_1,t_1;\vec{y},t_y) W_{\sigma,\tau}(\vec{x},t_x;\vec{y},t_y)
\end{eqnarray}


%*******************************************************************************************
%*******************************************************************************************
%*******************************************************************************************

\section{La TDDFT "rivestita"}

\subsection{Il problema di sistemi a shell aperta}


==> lavoro.tex <==
Cosa deve essere ancora fatto:
1 - Capitolo sulle approssimazioni  (4 gg)
2 - Capitolo dugli sviluppi per il kernel  (6 gg)
3 - Paragrafo risultati N_2 (1 gg)
4 - Introduzione (1 gg)
5 - Estensioni della teoria (paragrafi all'interno del lavoro di Casida) (1 gg)
6 - Inserire alcune delle correzioni di Onida

Dettagli da sistemare


==> vario.tex <==
\begin{table}[ht]
\begin{center}
\begin{tabular}{|l|l|l|l||l|}
\hline
Tipo di     & TDLDA      & TDLDA    &  Eccitazione & Presente              \\
eccitazione & Gaussian03 & DeMon2k  &  Principale  & Lavoro                \\
            &           &          &              & Abinit                \\  
\hline
$\Pi$     &  2.3657   &  2.2479  &  $3\sigma->1\pi\ \uparrow$           &  2.395             \\
$\Sigma$  &  4.6633   &  4.5103  &  $3\sigma->4\sigma\ \uparrow$        &  4.519             \\
$\Sigma$  &  4.7576   &  4.6300  &  $3\sigma->5\sigma\ \uparrow$        &  4.693             \\
$\Pi$     &  4.8451   &  4.7047  &  $3\sigma->2\pi\ \uparrow$           &  4.798             \\
$\Sigma$  &  5.1318   &  4.8049  &  $2\sigma->3\sigma\ \downarrow$      &  *****             \\
$\Pi$     &  5.6338   &  5.1685  &  $2\sigma->1\pi\ \uparrow\downarrow$ &  5.654             \\
$\Sigma$  &  5.6414   &  5.4803  &  $3\sigma->6\sigma\ \uparrow$        &  *****             \\
          &           &          &  $2\sigma->3\sigma\ \downarrow$      &                    \\
\hline
\end{tabular}
\caption{Spettro di eccitazione calcolate con il programma Abinit. Confronto
         con i risultati TDLDA riportati da Casida.
         Parametri: Acell 50 Bohr di raggio, nband 50, ecut 10 Hartree}
\rule{\linewidth}{0.2 mm}
\end{center}
\label{tab:eccitazioni-Abinit-1}
\end{table}


%**********************************************************************************************************
\begin{comment}
\subsection{Confronto con i risultati ottenuti da Casida}
Come abbiamo visto analizzando i dati ottenuti abbiamo un buon accordo con i dati riportati
da Casida \cite{Casida3} ma non siamo in grado di individuare la maggior parte delle eccitazioni
del sistema. Il problema ci spinge ad analizzare le differenze tra il nostro calcolo e il calcolo di
Casida e a cercare di capire come queste influenzino i valori per le eccitazioni con energia superiore
a $-\epsilon^{\uparrow}_{HOMO}$. In questo senso la principale differenza va individuata nel fatto che mentre
noi stiamo lavorando sviluppando le nostre funzioni d'onda in onde piane, Casida lavora sviluppando i conti
su di una base localizzata. Questo fa si che il vuoto venga trattato in modo differente nelle due sistuazioni.
Nel nostro caso dobbiamo necessariamente considerare una grande quantit\`{a} di spazio vuoto attorno alla
molecola e come conseguenza otteniamo una serie di stati con energie molto vicine tra loro che lo descrivono,
mentre per Casida sar\`{a}
sufficiente considerale una super cella di dimensioni pi\`{u} ridotte con il risultato di ottenere solo un
numero limitato di stati di vuoto.

Per capire ora come Casida possa individuare tra tutte le eccitazioni ottenute quelle valide ci rifacciamo al
lavoro esposto nella referenza \cite{Tesi_dot_Myrta}, in cui viene studiato lo spettro di eccitazione
della molecola $N_2$. Nel lavoro veengono confrontati
i risultati che si possono ottenere dalla TDDFT con differenti potenziali di
scambio e correlazione con i risultati che possono essere ottenuti con altri modelli teorici ed infine con
i dati sperimentali. In particolare in analogia a quanto fa Casida per lo studio della molecola di BeH viene
utilizzato un potenziale di scambio e correlazione con un andamento corretto nella regione asintotica,
il potenziale di ``van Leeuwen and Baerends'' \cite{Casida3} per il conto ground state.
Confrontando i diversi dati viene mostrato come lo spettro di eccitazioni che pu\`{o} essere calcolato
con la teoria TDDFT in approssimazione LDA risulta formato da una serie di energie di eccitazione che
non dovrebbero comparire e che l'autrice interpreta come dovuti appunto all'errore nella stima dell'energia
$\epsilon_{HOMO}$ e dunque alla presenza di stati di vuoto ``pi\`{u} vicini'' di quanto accada in realt\`{a}
agli stati di valenza. Poich\`{e} d'altra parte in tale lavoro viene utilizzata una base localizzata il numero
di eccitazioni di vuoto che compare risulta essere limitato e dunque, confrontando i dati 
con quelli ottenuti lavorando con un potenziale ad andamento corretto e con altri dati teorici,
si riesce ad individuare quali, tra le eccitazioni, vadano considerate come ``fisiche'' e quali
invece no.

Nel nostro caso invece il vuoto risulta descritto da una serie di stati con energie sempre pi\`{u}
vicine tra loro al crescere della dimensione della super-cella e dunque non riusciamo pi\`{u} ad individuare
le eccitazioni fisiche, come invece probabilmente \`{e} in grado di fare Casida il quale si troverebbe,
supponiamo, a lavorare comunque con un numero di eccitazioni ``di vuoto'' limitato.

Ci\`{o} che comunque possiamo fare \`{e} considerare, oltre alle eccitazioni con energia inferiore a
$-\epsilon^{\uparrow}_{HOMO}$, tutte le eccitazioni che compaiono tra stati di valenza,
ovvero che coinvolgono i primi cinque stati del nostro sistema ($2\sigma$, $3\sigma$, $1\pi$ e
$4\sigma$), che sono poi le stesse che nel grafico (fig.\ref{fig:BeH_convergenza}) sono a convergenza
anche rispetto alle dimensioni della super-cella.
I risultati che otteniamo sono dunque i seguenti nella tabella (\ref{tab:eccitazioni_all})

\begin{table}[!ht]
\begin{center}
\begin{tabular}{|l|l|l|l|l|}
\hline
Eccitazione  &  energia  & eccitazione & Configurazione & Contributo                        \\
             &           & principale  & elettronica    & dell'eccitazione                  \\
             &           &             &                & principale                         \\
\hline
$\Pi$    & 2.398 & $3\sigma\rightarrow 1\pi\ \uparrow$           & $2\sigma^2 1\pi^1$              & 99\% \\
$\Sigma$ & 4.534 & $3\sigma\rightarrow 4\sigma\ \uparrow$        & $2\sigma^2 4\sigma^1$           & 99\% \\
$\Sigma$ & 5.536 & $2\sigma\rightarrow 3\sigma\ \downarrow$      & $2\sigma^1 3\sigma^2$           & 96\% \\
$\Pi$    & 5.657 & $2\sigma\rightarrow 1\pi\ \uparrow\downarrow$ & $2\sigma^1 3\sigma^1 1\pi^1$    & 99\% \\
$\Pi$    & 7.145 & $2\sigma\rightarrow 1\pi\ \uparrow\downarrow$ & $2\sigma^1 3\sigma^1 1\pi^1$    & 97\% \\
$\Sigma$ & 7.962 & $2\sigma\rightarrow 4\sigma\ \downarrow$      & $2\sigma^1 3\sigma^1 4\sigma^1$ & 99\% \\
$\Sigma$ & 8.277 & $2\sigma\rightarrow 4\sigma\ \uparrow$        & $2\sigma^1 3\sigma^1 4\sigma^1$ & 52\% \\
\hline
\end{tabular}
\caption{Schema completo delle eccitazioni a convergenza, le eccitazioni sono state
         scelte osservando i grafici in figura (\ref{fig:BeH_convergenza})
         I parametri dei risultati riportati sono acell 70, ecut 10, nband 50}
\rule{\linewidth}{0.2 mm}
\end{center}
\label{tab:eccitazioni_all}
\end{table}

Se ora cerchiamo di confrontare i dati del presente lavoro con i dati della referenza \cite{Casida3}
possiamo inserire le eccitazioni come fatto nella tabella (\ref{tab:eccitazioni_Casida}).

\begin{table}[!ht]
\begin{center}
\begin{tabular}{|l|l|l|l|}
\hline
Eccitazione  &  Presente & Casida  &  Dati teorici            \\
             &  lavoro   &         &  PTN                     \\
\hline
$1\Pi$       &  2.398    &  2.391  &  2.56                    \\
$2\Sigma$    &  4.534    &  4.593  &  5.51                    \\
$3\Sigma$    &           &  4.771  &  5.61                    \\
$4\Sigma$    &           &  5.129  &  6.12                    \\
$2\Pi$       &           &  4.858  &  6.31                    \\
$5\Sigma$    &  5.536    &  5.418  &  6.71                    \\
$3\Pi$       &  5.657    &  5.671  &  6.74                    \\
$4\Pi$       &           &  5.732  &  7.27                    \\
$\Pi$        &  7.145    &         &                          \\
$\Sigma$     &  7.962    &         &                          \\
$\Sigma$     &  8.277    &         &                          \\
\hline
\end{tabular}
\caption{Raffronto tra le energie di eccitazione ottenute nel presente lavoro e quelle ottenute
         da Casida nell'articolo \cite{Casida3}}
\rule{\linewidth}{0.2 mm}
\end{center}
\label{tab:eccitazioni_Casida}
\end{table}

Le eccitazioni del presente lavoro sono state inserite in tabella cercando di riprodurre i risultati
di Casida, d'altra parte non abbiamo alcun riferimento che ci permetta di individuare a quali delle
eccitazioni indicate possa corrispondere il nostro risultato se non la distinzione $\Pi$, $\Sigma$.
Ancora una volta, ad ogni modo, abbiamo un buon accordo tra i nostri dati e quelli di Casida, il che
rafforza le nostre convinzioni che i calcoli da noi svolti siano probabilmente fatti nel modo corretto.


%************************************************************************************************************
\subsection{Un'analisi pi\`{u} sistematica dei nostri risultati}

Fino ad ora abbiamo lavorato tenendo come punto di riferimento le energie di eccitazione della referenza
\cite{Casida3}
poich\'{e} calcolate nell'ambito della stessa teoria da noi utilizzata. Ci siamo poi in particolare concentrati
sul fatto che i conti svolti partendo da un calcolo ground state LDA portino ad una sottostima del valore
$-\epsilon^{\uparrow}_{HOMO}$ ed abbiamo cercato di individuare un modo per superare questo problema facendo in
particolare riferimento al lavoro \cite{Tesi_dot_Myrta}.

Non abbiamo per\`{o} in alcun modo tenuto in
considerazione i problemi di cui abbiamo parlato presentando la formulazione di Casida per la TDDFT per sistemi
con stato fondamentale a spin polarizzato. In effetti anche nel lavoro \cite{Casida3} questo problema non
sembra essere tenuto in considerazione (segnaliamo che la pubblicazione del lavoro \cite{Casida3}
precede di circa 5 anni la pubblicazione del lavoro \cite{Casida2} in cui si parla di tale problema) poich\'{e}
in tale lavoro vengono presentate tutte le eccitazioni della molecola, mentre sappiamo che la nostra teoria, in
approssimazione adiabatica, in
principio non \`{e} in grado di prevedere alcune delle eccitazioni, in particolare le eccitazioni
a particella doppia.

Sorge dunque il dubbio che nell'analizzare le energie di eccitazioni gli autori della
referenza \cite{Casida3} abbiano considerato in modo errato anche il problema degli stati di vuoto
ottenendo cos\`{i} le eccitazioni mancanti nella teoria proprio da eccitazioni verso stati di vuoto.
Crediamo quindi un punto di partenza migliore per l'analisi dei nostri dati abbandonare il confronto
con tale referenza e cercare di sviluppare una nuova interpretazione.

Ricordiamo dunque
che in base a quanto gi\`{a} detto un calcolo eseguito nell'ambito di un sistema spin-polarizzato
dovrebbe essere in gradi di prevedere in modo corretto solo quelle eccitazioni che conservano $S^2$.
Questo problema in particolare compare per tutte quelle eccitazioni verso stati che presentano tre bande
parzialmente occupate. Tra queste,
per poter scegliere quali siano tra le eccitazioni da noi calcolate quelle che conservano lo spin totale del
sistema, possiamo far riferimento alla regola di Hund e all'analisi della configurazione elettronica dello
stato eccitato. Se infatti consideriamo due eccitazioni che presentano la medesima configurazione elettronica,
dal punto di vista spaziale,
possiamo individuare come stati di doppietto quelli con energia di eccitazione maggiore, mentre come stati di
tripletto/quadripletto quello con energia di eccitazione minore. Poich\'{e} infine lo stato fondamentale del
nostro sistema \`{e} un doppietto la regole risulta che date due energie di eccitazione verso due stati
che presentano
la medesima configurazione elettronica spaziale dobbiamo considerare solo l'eccitazione ad energia maggiore.

Teniamo dunque in considerazione questa ulteriore regola nell'analisi dei nostri dati.
Infine teniamo conto del problema della stima di $-\epsilon^{\uparrow}_{HOMO}$ scegliendo di considerare solo
quelle eccitazioni
che coinvolgono i livelli con autovalore lontano dal livello di vuoto (stati: $2\sigma$, $3\sigma$, e $1\pi$)
scartando quindi anche le eccitazioni verso lo stato $4\sigma$.
In questo modo ci restano solo tre eccitazioni che, confrontate con dati sperimentali e altri dati teorici danno
per\`{o} un ottimo accordo, come mostrato nella tabella (\ref{tab:eccitazioni_finale}).

\begin{table}[!ht]
\begin{center}
\begin{tabular}{|l||l|l||l|l|}
\hline
Eccitazione  & Dati     & Dati    & Presente & Dati teorici  \\
             & sperim.  & sperim. & lavoro   & PTN           \\
\hline
$1\Pi$       &  2.484   &  2.48   &   2.398  & 2.56          \\
$2\Sigma$    &          &         &   5.536  & 5.51          \\
$3\Sigma$    &          &         &          & 5.61          \\
$4\Sigma$    &          &  6.06   &          & 6.12          \\
$2\Pi$       &  6.317   &  6.31   &          & 6.31          \\
$5\Sigma$    &          &  6.70   &          & 6.71          \\
$3\Pi$       &          &         &          & 6.74          \\
$4\Pi$       &  7.460   &  7.28   &   7.145  & 7.27          \\
\hline
\end{tabular}
\caption{Raffronto tra le energie di eccitazione ottenute nel presente lavoro
         e dati sperimentali e teorici presi dalle referenze \cite{Casida3} e
         \cite{PTN_BeH}}
\rule{\linewidth}{0.2 mm}
\end{center}
\label{tab:eccitazioni_finale}
\end{table}

Ricordiamo ancora una volta che in effetti lo scegliere per un valore ottenuto una determinata eccitazione
sia stato fatto in modo arbitrario, non avendo, dalle referenze, alcuna indicazione in proposito.
Oltre all'ottimo accordo con i dati
sperimentali, a nostro avviso, un grande vantaggio \`{e} costituito dal fatto che questa interpretazione
coinvolge principalmente i primi stati del sistema e giustifica quindi l'utilizzo di super-celle di dimensioni
pi\`{u} limitate. In particolare se guardiamo alla figura (\ref{fig:BeH_convergenza}) vediamo che le
eccitaizoni sche abbiamo scelto (ovvero quelle che coinvolgono gli stati $2\sigma$, $3\sigma$, e $1\pi$)
sono le meno sensibili alle dimensioni della super-cella. La scelta di scartare lo stato $4\sigma$ pu\`{o}
inoltre essere motivata osservando le immagini delle funzioni d'onda per i diversi orbitali riportati alla
fine di questo capitolo. In particolare si vede che i due orbitali ($4\sigma\uparrow$) e ($4\sigma\downarrow$)
che sono mostrati nella serie di immagini (\ref{fig:BeH_vacuum_5up}) e (\ref{fig:BeH_vacuum_5down}) presentano
un andamento molto pi\`{u} simile a quello di un orbitale di vuoto (\ref{fig:BeH_vacuum_6up}) che non a quelle
degli ``orbitali fisici''.

Concludiamo l'analisi dei dati sottolineando come nel lavoro svolto le due approssimazioni eseguite,
l'approssimazione LDA
(e quindi l'errato andamento del potenziale di scambio e correlazione nella regione asintotica) per
il computo dello stato fondamentale e l'approssimazione adiabatica
per il computo del kernel hanno portato come conseguenza il
fatto che non siamo in grado di individuare la maggior parte delle eccitazioni del sistema. Sui tentativi
di migliorare l'approssimazione LDA abbiamo visto come una soluzione viene presentata in particolare
nella referenza \cite{Tesi_dot_Myrta} e crediamo che tale problema sia stato gi\`{a} studiato in molte
altre occasioni nel computo dello stato fondamentale di differenti sistemi e ben delineato. Dal nostro
punto di vista crediamo possa essere un obiettivo di non difficile difficolt\`{a} implementare una delle
possibili soluzioni all'interno del programma da noi utilizzato nell'ambito di questa tesi.

Il problema del miglioramento dell'approssimazione adiabatica invece \`{e} ad oggi uno degli argomenti di cui
si occupa la ricerca. Abbiamo dunque scelto di mostrare, nel prossimo capitolo, due possibili approcci che
permetterebbero di giungere alla soluzione di tale difficolt\`{a} e che sono presi rispettivamente dalle
referenze \cite{Casida2} e \cite{Tesi_dot_Fabien},\cite{Fabien_kernel}. Dal nostro punto di vista
l'implementazione di una di questi due soluzioni resta una sfida di maggiore difficolt\`{a}.
\end{comment}


%******************************************************************************************************************
%******************************************************************************************************************
%******************************************************************************************************************
\begin{comment}
Una grazie ai professori e alle persone che mi hanno seguito in questo lavoro di tesi
per circa un anno, per l'entusiasmo nel fare le cose del professor Gonze (many thanks!),
per la puntualit\`{a} e la disponibilit\`{a} del professor Rignanese, per le numerose
indicazioni ricevute da Nicola Manini e infine per i piccoli ma preziosi aiuti ricevuti
da Lucia.
Soprattutto una nota speciale per il professor Onida perch\`{e} questo lavoro di tesi 
\`{e} stato reso possibile soprattutto grazie alla sua disponibilit\`{a} a partire dal
tempo dedicato per trovare un lavoro di tesi che soddisfasse le mie richieste, passando 
per l'avermi messo in contatto con i professori che mi hanno seguito durante il
periodo trascorso in Belgio, con il progetto Abinit e con il ``mondo nanoquanta'',
e in ultimo per aver trovato una borsa di studio che lo sostenesse.
D'altra parte chi mi sta vicino mi avr\`{a} spesso sentito lamentarmi perch\'{e} questo
o quello non andava bene; riguardando il lavoro svolto la sensazione
che provo \`{e} quella di aver perso una grande quantit\`{a} di tempo ad occuparmi di
questioni che affrontate in modo differente avrebbero certo richiesto un dispendio minore di
energie. La ragione di questo credo dipenda in parte dal fatto che, soprattutto quando si
tratta di fisica, tendo a voler fare le cose di testa mia, in parte dal modo in cui il tutto
\`{e} stato gestito sin dall'inizio. Il risultato \`{e} stato 
un anno di lavoro intenso e spesso, a mio avviso, troppo
caotico. Non so se esista un modo migliore di quello percorso per affrontare le cose ma certo
se dovessi ricominciare tutto da capo tenterei di organizzarmi in modo differente.
\end{comment}



\begin{comment}
%*********************************************************************************************
%*********************************************************************************************
%*********************************************************************************************
\section*{I contenuti di questo lavoro}

La scelta di questo campo della fisica (la fisica della materia), piuttosto che della
fisica teorica, che ritengo comunque la specializzazione pi\`{u} affascinante, \`{e}
stata dettata da molte ragioni,tra le quali anche ragioni di natura pratica e di
opportunit\`{a}.
Uno dei motivi pi\`{u} profondi resta comunque il fatto che ero curioso di dedicarmi
ad un lavoro che si avvicinasse il pi\`{u} possibile ad un'applicazione nella realt\`{a},
seppur rimanendo nell'ambito di una tesi di tipo teorico e non sperimentale.

Il fatto che questo lavoro sia definito una tesi di tipo teorico significa che ci
concentreremo sullo studio di uno dei modelli matematici che vengono utilizzati
dai fisici per descrivere la realt\`{a} e cercheremo, nel nostro piccolo, di
sviluppare ulteriormente le possibilit\`{a} di tale modello.

Pi\`{u} in dettaglio in questo lavoro siamo interessati al calcolo dello spettro di
eccitazione di un materiale ed sar\`{a} proprio cercare di prevedere tale spettro
lo scopo del nostro modello.
\\
fare riferimento alla pubblicazione di Onida \\
\\

Ci\`{o} che per\`{o} vi \`{e} di straordinario nei
conti che faremo in questa tesi, e che sono gli stessi che molte persone che studiano
fisica della materia fanno, sar\`{a} il fatto che per ottenere il nostro scopo verranno
utilizzati modelli in grado di calcolare il comportamento di un numero enorme di elettroni,
quale \`{e} quello che costituisce un qualsiasi oggetto di dimensioni macroscopiche.
Dico questo per farvi capire come sebbene i fisici, come abbiamo gi\`{a} spiegato,
non riescano ancora certo a spiegare tutto a partire dalle sole leggi universali che
regolano le particelle elementari, certo sono riusciti in questi anni
ad ottenere risultati straordinari.

Il modello matematico che dovremo utilizzare per i nostri scopi sar\`{a} quello della
meccanica quantistica di cui parleremo nell'ultima sezione di questa introduzione.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\subsection*{La meccanica quantistica e altro, sempre per i non addetti ai lavori}
Insieme alla teoria della relativit\`{a} la meccanica quantistica rappresenta l'altra
grande rivoluzione che agli inizi del '900 ha cambiato il modo in cui i fisici
guardano alla realt\`{a} che ci circonda. A differenza della teoria della relativit\`{a}
per\`{o} la meccanica quantistica resta a tutt'oggi semplicemente un modello e
non una teoria chiusa. Ci\`{o} significa in altre parole che questo il modello matematico,
che viene utilizzato per cercare di descrivere la realt\`{a} microscopica,
non \`{e} stato ancora completamente compreso e che non \`{e} in grado di descrivere
appieno tale realt\`{a}.

In una delle sezioni precedenti abbiamo affermato che uno dei motivi per cui la fisica
non arriver\`{a} mai a poter spiegare entit\`{a} complesse quali le cellule che sono
alla base della vita dipende dal fatto che neanche le particelle pi\`{u} semplici si
comportano in modo deterministico. Questo fatto costituisce probabilmente
il cuore della meccanica quantistica; secondo tale modello infatti non \`{e} possibile
determinare in modo esatto la traiettoria di una particella ma semplicemente \`{e}
possibile stabilire la probabilit\`{a} che questa si comporti in una determinata maniera.
Ci\`{o} che realmente accade \`{e} lasciato al caso e non pu\`{o} in alcun modo
essere controllato dai fisici al di l\`{a} di quanto la meccanica quantistica \`{e}
in grado di fare.
Per questa ragione dunque la fisica non pu\`{o} essere in grado di ridurre il nostro
universo ad un semplice fenomeno meccanico e dunque di svuotare la realt\`{a}, o
perlomeno il nostro modo di concepirla, di quell'idea di spiritualit\`{a}
a cui molte persone credono profondamente.

Il fatto che a tutt'oggi la meccanica quantistica non sia stata ancora compresa
appieno e che essa non sia in grado di descrivere in modo deterministico non significa
per\`{o} che tale modello sia qualcosa a cui si debba guardare con un certo sospetto.
Sin da quando \`{e} stato elaborato agli inizi del novecento esso \`{e} stato infatti
in grado di prevedere correttamente tutti i risultati degli esperimenti che fisici 
e non hanno da allora realizzato. Anche in questa tesi ci serviremo dunque di questo 
modello e, sebbene non li potrete comprendere, spero guardiate a questi risultati
come a un qualcosa di valido poich\'{e} basato su un modello matematico che \`{e}
stato verificato infinite volte. Potrete certo dubitare sulle interpretazioni
che possono essere date riguardo al comportamento delle particelle, ma non
degli strumenti utilizzati per il calcolo, per quanto essi possano apparire
oscuri e lontani dal nostro modo di guardare alla realt\`{a} che ci circonda.


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\end{comment}




